Migrating Software Systems towards Post-Quantum-Cryptography -- A Systematic Literature Review

Networks such as the Internet are essential for our connected world. Quantum computing poses a threat to this heterogeneous infrastructure since it threatens fundamental security mechanisms. Therefore, a migration to post-quantum-cryptography (PQC) is necessary for networks and their components. At the moment, there is little knowledge on how such migrations should be structured and implemented in practice. Our systematic literature review addresses migration approaches for IP networks towards PQC. It surveys papers about the migration process and exemplary real-world software system migrations. On the process side, we found that terminology, migration steps, and roles are not defined precisely or consistently across the literature. Still, we identified four major phases and appropriate substeps which we matched with also emerging archetypes of roles. In terms of real-world migrations, we see that reports used several different PQC implementations and hybrid solutions for migrations of systems belonging to a wide range of system types. Across all papers we noticed three major challenges for adopters: missing experience of PQC and a high realization effort, concerns about the security of the upcoming system, and finally, high complexity. Our findings indicate that recent standardization efforts already push quantum-safe networking forward. However, the literature is still not in consensus about definitions and best practices. Implementations are mostly experimental and not necessarily practical, leading to an overall chaotic situation. To better grasp this fast moving field of (applied) research, our systematic literature review provides a comprehensive overview of its current state and serves as a starting point for delving into the matter of PQC migration.

==> tables/03_hybrid_migration.tex <==
\begin{table}
\small
  \centering
  \caption{The approach of the analyzed papers regarding hybrid migration
    strategies.\label{t:hybrid_migration}}
  \begin{tabular}{cccc}
    \toprule
	\textbf{Ref} & \textbf{Claimed} & \textbf{Recommended} & \textbf{Mentioned} \\
	\midrule
	\citer{caraf} & & & \\
	\citer{cyber} & & & \textbullet \\
	\citer{impact_hybrid} & \textbullet & & \\
	\citer{microservice} & \textbullet & & \\
	\citer{tls_database} & \textbullet & & \\
	\citer{ibe} & & & \textbullet \\
	\citer{ibm_db2} & & & \\
	\citer{dep_analysis} & & & \textbullet \\
	\citer{nist_migration} & & & \textbullet \\
	\citer{making_decisions} & \textbullet & \textbullet & \\
	\citer{nginx_migration} & & & \\
	\citer{hbs_iot} & & \textbullet & \\
	\citer{pmmp} & & & \\
	\citer{pqc_ros} & \textbullet & & \\
	\citer{pqfabric} & & & \\
	\citer{pqc_email} & & & \textbullet \\
	\citer{cits} & & & \textbullet \\
	\citer{refine_mosca} & & \textbullet & \\
	\citer{complex_path} & & \textbullet & \\
	\citer{handbook} & \textbullet & & \\
	\bottomrule
  \end{tabular}
\end{table}


==> tables/id.tex <==
\begin{table}
\small
  \centering
  \caption{List of all analyzed papers with their publication year. \label{t:id}}
  \begin{tabular}{cp{6cm}c}
    \toprule
		\textbf{Ref} & \textbf{Title} & \textbf{Year}\\
	\midrule \\
		\citer{caraf} & CARAF: Crypto Agility Risk Assessment Framework & 2021\\
		\citer{cyber} & CYBER; Migration strategies and recommendations to Quantum Safe
		schemes & 2020\\
		\citer{impact_hybrid} & Impact of post-quantum hybrid certificates on PKI, common
		libraries, and protocols & 2021\\
		\citer{microservice} & Incorporating post-quantum cryptography in a microservice
		environment & 2020\\
		\citer{tls_database} & Integrating and Evaluating Quantum-safe TLS in Database
		Applications & 2022\\
		\citer{ibe} & Identity-Based Encryption A Comparison of Leading Classical and
		Post-Quantum Implementations in an Enterprise Setting & 2022\\
		\citer{ibm_db2} & Making existing software quantum safe: a case study on IBM Db2
	  & 2023\\
		\citer{dep_analysis} & Migrating to Post-Quantum Cryptography: a Framework Using
		Security Dependency Analysis & 2023\\
		\citer{nist_migration} & MIGRATION TO POST-QUANTUM CRYPTOGRAPHY & 2021\\
		\citer{making_decisions} & Migration to quantum-safe cryptography: about making
		decisions on when, what and how to migrate to a quantum-safe situation & 2020\\
		\citer{nginx_migration} & Migrating Nginx Web Servers to Quantum-Safe TLS &
		2021\\
		\citer{hbs_iot} & On the Role of Hash-Based Signatures in Quantum-Safe Internet
		of Things: Current Solutions and Future Directions & 2021\\
		\citer{pmmp} & PMMP - PQC Migration Management Process & 2023\\
		\citer{pqc_ros} & Post Quantum Secure Command and Control of Mobile Agents &
		2020\\
		\citer{pqfabric} & PQFabric: A Permissioned Blockchain Secure from Both Classical
		and Quantum Attacks & 2021\\
		\citer{pqc_email} & Quantum-resistant End-to-End Secure Messaging and Email
		Communication & 2023\\
		\citer{cits} & Quantum-Safe Cryptography (QSC) Migration; ITS and C-ITS migration
		study & 2023\\
		\citer{refine_mosca} & Refining Mosca’s Theorem: Risk Management Model for the
		Quantum Threat Applied to IoT Protocol Security & 2022\\
		\citer{complex_path} & The Complex Path to Quantum Resistance & 2021\\
		\citer{handbook} & The PQC Migration handbook & 2023\\
		\citer{ibm_z} & Transitioning to Quantum-Safe Cryptography on IBM Z & 2022\\
	\bottomrule
  \end{tabular}
\end{table}

